Masked Faces with Faced Masks

Modern face recognition systems (FRS) still fall short when the subjects are wearing facial masks, a common theme in the age of respiratory pandemics. An intuitive partial remedy is to add a mask detector to flag any masked faces so that the FRS can act accordingly for those low-confidence masked faces. In this work, we set out to investigate the potential vulnerability of such FRS equipped with a mask detector, on large-scale masked faces, which might trigger a serious risk, e.g., letting a suspect evade the FRS where both facial identity and mask are undetected. As existing face recognizers and mask detectors have high performance in their respective tasks, it is significantly challenging to simultaneously fool them and preserve the transferability of the attack. We formulate the new task as the generation of realistic & adversarial-faced mask and make three main contributions: First, we study the naive Delanunay-based masking method (DM) to simulate the process of wearing a faced mask that is cropped from a template image, which reveals the main challenges of this new task. Second, we further equip the DM with the adversarial noise attack and propose the adversarial noise Delaunay-based masking method (AdvNoise-DM) that can fool the face recognition and mask detection effectively but make the face less natural. Third, we propose the adversarial filtering Delaunay-based masking method denoted as MF2M by employing the adversarial filtering for AdvNoise-DM and obtain more natural faces. With the above efforts, the final version not only leads to significant performance deterioration of the state-of-the-art (SOTA) deep learning-based FRS, but also remains undetected by the SOTA facial mask detector, thus successfully fooling both systems at the same time.

==> ACMMM22_FaceMask/misc_IJCAI/table1.tex <==
\begin{table}[]
% \footnotesize
\scriptsize
    \centering
    \label{tab:mask_detection}
    \caption{Multifaceted evaluation of each masking method.}
    \vspace{-3pt}
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \setlength{\tabcolsep}{3pt}
    % \resizebox{1\linewidth}{!}{
    \begin{tabular}{ccccc}
    \hline
    % \toprule 
        & Solid-color & DM & AdvNoise-DM (ours) & $\text{MF}^2\text{M}$ (ours) \tabularnewline
    % \midrule
    \hline
     AUC & 0.9987 & 0.9956 & 0.4163 & {0.4093} \tabularnewline
     Mask Rate & 90.53\% & 27.74\% & 7.30\% & {6.95\%} \tabularnewline
     SSIM & — & — & 0.9808 & {0.9812} \tabularnewline
     PSNR & — & — & 38.76 & {40.45} \tabularnewline
    % \bottomrule 
    \hline
    \end{tabular}
    % }
    \label{Table:table}
    % \vspace{2pt}
\end{table}

==> ACMMM22_FaceMask/physical_black.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \vspace{-3pt}
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of \textit{physical} black-box attacks. 
"Rank 1" refers to the top-1 identification rate and "Veri." refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
\hline 
 & \multicolumn{3}{c|}{CosFace ResNet50} & \multicolumn{3}{c}{CosFace ResNet34}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Face Rec. & \multicolumn{2}{c|}{\cellcolor{gray!40}Face Verification} & Face Rec. & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & AUC & Rank 1 & Veri. & AUC\tabularnewline
\hline 
Solid-color (phys.) & 0.7740 & 0.7846 & 0.9992 & 0.7586 & 0.7670 & 0.9993\tabularnewline
DM (phys.) & 0.7527 & 0.7369 & 0.9987 & 0.6757 & 0.6739 & 0.9985\tabularnewline
I-FGSM (phys.) & 0.6686 & 0.6791 & 0.9958 & 0.6734 & 0.6438 & 0.9951\tabularnewline
\hline 
\textbf{AdvNoise-DM (phys.)} & 0.2189 & 0.2184 & 0.9683 & 0.1858 & 0.1860 & 0.9627\tabularnewline
\textbf{$\text{MF}^{2}\text{M}$ (phys.)} & \textbf{0.1692} & \textbf{0.1818} & \textbf{0.9670} & \textbf{0.1633} & \textbf{0.1336} & \textbf{0.9498}\tabularnewline
\hline 
\end{tabular}
}


\label{Table:physical_black}

\vspace{10pt}

\end{table}

==> ACMMM22_FaceMask/physical_white.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \vspace{-3pt}
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of \textit{physical} white-box attacks. 
"Rank 1" refers to the top-1 identification rate and "Veri." refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline 
 & \multicolumn{1}{c}{Face Rec.} & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification} & \multicolumn{1}{c}{Mask Detection}\tabularnewline
\hline 
 & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Mask Rate}\tabularnewline
\hline 
Solid-color (phys.)& 0.7302 & 0.7398 & 0.9985 & 100\%\tabularnewline
DM (phys.)& 0.5574 & 0.5550 & 0.9975 & 10\%\tabularnewline
I-FGSM (phys.)& 0.2284 & 0.2497 & 0.9453 & 95\%\tabularnewline
\hline 
\textbf{AdvNoise-DM (phys.)} & \textbf{0.0000} & \textbf{0.0000} & 0.6879 & \textbf{10\%}\tabularnewline
\textbf{$\text{MF}^{2}\text{M}$ (phys.)} & \textbf{0.0000} & \textbf{0.0000} & \textbf{0.6658} & \textbf{10\%}\tabularnewline
\hline 
\end{tabular}
}
\vspace{10pt}



\label{Table:physical_white}

\vspace{5pt}

\end{table}

==> ACMMM22_FaceMask/table_black.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of each masking method on black-box attack.
``Rank 1'' refers to the top-1 identification rate and ``Veri.'' refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
   \begin{tabular}{l|ccc|ccc}
\hline 
 & \multicolumn{3}{c|}{CosFace ResNet50} & \multicolumn{3}{c}{CosFace ResNet34}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Face Rec. & \multicolumn{2}{c|}{\cellcolor{gray!40}Face Verification} & Face Rec. & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Rank 1 & Veri. & AUC & Rank 1 & Veri. & AUC\tabularnewline
\hline 
Solid-color & 0.8207 & 0.8233 & 0.9991 & 0.7641 & 0.7697 & 0.9987\tabularnewline
\hline 
FGSM & 0.7585 & 0.7624 & 0.9988 & 0.7147 & 0.7212 & 0.9984\tabularnewline
I-FGSM & 0.6720 & 0.6752 & 0.9978 & 0.6243 & 0.6303 & 0.9967\tabularnewline
MI-FGSM & 0.6419 & 0.6445 & 0.9972 & 0.6020 & 0.6077 & 0.9961\tabularnewline
TI-FGSM & 0.7640 & 0.7711 & 0.9988 & 0.7142 & 0.7214 & 0.9984\tabularnewline
TI-MI-FGSM & 0.6416 & 0.6438 & 0.9972 & 0.5996 & 0.6038 & 0.9958\tabularnewline
$\text{DI}^2$-FGSM & 0.7178 & 0.7222 & 0.9983 & 0.6699 & 0.6777 & 0.9977\tabularnewline
M-$\text{DI}^2$-FGSM & 0.6559 & 0.6592 & 0.9974 & 0.6165 & 0.6242 & 0.9963\tabularnewline
\hline 
\textbf{DM (ours)} & 0.6400 & 0.6520 & 0.9971 & 0.5987 & 0.6126 & 0.9971\tabularnewline
\textbf{AdvNoise-DM (ours)} & 0.0726 & 0.0723 & 0.9293 & 0.0657 & 0.0622 & 0.9310\tabularnewline
\textbf{$\text{MF}^2\text{M}$ (ours)} & \textbf{0.0674} & \textbf{0.0670} & \textbf{0.9237} & \textbf{0.0546} & \textbf{0.0508} & \textbf{0.9212}\tabularnewline
\hline 
\end{tabular}
}

\label{Table:table_black}

\vspace{5pt}

\end{table}

==> ACMMM22_FaceMask/table_white.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \vspace{-3pt}
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of each masking method on white-box attack. 
"Rank 1" refers to the top-1 identification rate and "Veri." refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l|cccc}
\hline 
 & \multicolumn{1}{c}{Face Rec.} & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification} & \multicolumn{1}{c}{Mask Detection}\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}
 & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Mask Rate} \tabularnewline
\hline 
Solid-color & 0.7389 & 0.7470 & 0.9986 & 90.53\%  \tabularnewline
\hline 
FGSM & 0.4895 & 0.4924 & 0.9950 & 62.10\%  \tabularnewline
I-FGSM & 0.0039 & 0.0026 & 0.7594 & 39.41\%  \tabularnewline
MI-FGSM & 0.0179 & 0.0135 & 0.8667 & 43.91\%  \tabularnewline
TI-FGSM & 0.4991 & 0.5053 & 0.9950 & 66.00\%  \tabularnewline
TI-MI-FGSM & 0.0364 & 0.0290 & 0.8998 & 51.97\%  \tabularnewline
$\text{DI}^2$-FGSM & 0.0690 & 0.0601 & 0.9193 & 43.51\%  \tabularnewline
M-$\text{DI}^2$-FGSM & 0.0705 & 0.0623 & 0.9293 & 45.50\% \tabularnewline
\hline
\textbf{DM (ours)} & 0.5146 & 0.5154 & 0.9956 & 27.74\%  \tabularnewline
\textbf{AdvNoise-DM (ours)} & \textbf{1.35$\text{e}^{-5}$} & \textbf{1.35$\text{e}^{-5}$} &  0.4163 & 7.30\% \tabularnewline
\textbf{$\text{MF}^2\text{M}$ (ours)} & \textbf{1.35$\text{e}^{-5}$} & 2.02$\text{e}^{-5}$ & \textbf{0.4093} & \textbf{6.95\%} \tabularnewline
\hline

%   \begin{tabular}{l|cccccc}
% \hline 
%  & \multicolumn{1}{c}{Face Recognition} & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification} & \multicolumn{1}{c}{Mask Detection} & \multicolumn{2}{c}{\cellcolor{gray!40}Similarity Metrics}\tabularnewline
% \cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
%  & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Mask Rate} & \multicolumn{1}{c}{SSIM} & PSNR\tabularnewline
% \hline 
% Solid-color & 0.7389 & 0.7470 & 0.9986 & 90.53\% & —&— \tabularnewline
% \hline 
% FGSM & 0.4895 & 0.4924 & 0.9950 & 62.10\% & — & —\tabularnewline
% I-FGSM & 0.0039 & 0.0026 & 0.7594 & 39.41\% & — & — \tabularnewline
% MI-FGSM & 0.0179 & 0.0135 & 0.8667 & 43.91\% & — & — \tabularnewline
% TI-FGSM & 0.4991 & 0.5053 & 0.9950 & 66.00\% & — & — \tabularnewline
% TI-MI-FGSM & 0.0364 & 0.0290 & 0.8998 & 51.97\% & — & — \tabularnewline
% $\text{DI}^2$-FGSM & 0.0690 & 0.0601 & 0.9193 & 43.51\% &  — & — \tabularnewline
% M-$\text{DI}^2$-FGSM & 0.0705 & 0.0623 & 0.9293 & 45.50\% & — & —\tabularnewline
% \hline
% \textbf{DM (ours)} & 0.5146 & 0.5154 & 0.9956 & 27.74\% & — & — \tabularnewline
% \textbf{AdvNoise-DM} (ours) & \textbf{1.35$\text{e}^{-5}$} & \textbf{1.35$\text{e}^{-5}$} &  0.4163 & 7.30\% & 0.9808 & 38.76\tabularnewline
% \textbf{$\text{MF}^2\text{M}$} (ours) & \textbf{1.35$\text{e}^{-5}$} & 2.02$\text{e}^{-5}$ & \textbf{0.4093} & \textbf{6.95\%} & 0.9812 & 40.45 \tabularnewline
% \hline


\end{tabular}
}


\label{Table:table_white}

\vspace{5pt}

\end{table}

==> FaceMask/physical_black.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \vspace{-3pt}
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of \textit{physical} black-box attacks. 
"Rank 1" refers to the top-1 identification rate and "Veri." refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
\hline 
 & \multicolumn{3}{c|}{CosFace ResNet50} & \multicolumn{3}{c}{CosFace ResNet34}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Face Rec. & \multicolumn{2}{c|}{\cellcolor{gray!40}Face Verification} & Face Rec. & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & AUC & Rank 1 & Veri. & AUC\tabularnewline
\hline 
Solid-color (phys.) & 0.7740 & 0.7846 & 0.9992 & 0.7586 & 0.7670 & 0.9993\tabularnewline
DM (phys.) & 0.7527 & 0.7369 & 0.9987 & 0.6757 & 0.6739 & 0.9985\tabularnewline
I-FGSM (phys.) & 0.6686 & 0.6791 & 0.9958 & 0.6734 & 0.6438 & 0.9951\tabularnewline
\hline 
\textbf{AdvNoise-DM (phys.)} & 0.2189 & 0.2184 & 0.9683 & 0.1858 & 0.1860 & 0.9627\tabularnewline
\textbf{$\text{MF}^{2}\text{M}$ (phys.)} & \textbf{0.1692} & \textbf{0.1818} & \textbf{0.9670} & \textbf{0.1633} & \textbf{0.1336} & \textbf{0.9498}\tabularnewline
\hline 
\end{tabular}
}


\label{Table:physical_black}

\vspace{10pt}

\end{table}

==> FaceMask/physical_white.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \vspace{-3pt}
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of \textit{physical} white-box attacks. 
"Rank 1" refers to the top-1 identification rate and "Veri." refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline 
 & \multicolumn{1}{c}{Face Rec.} & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification} & \multicolumn{1}{c}{Mask Detection}\tabularnewline
\hline 
 & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Mask Rate}\tabularnewline
\hline 
Solid-color (phys.)& 0.7302 & 0.7398 & 0.9985 & 100\%\tabularnewline
DM (phys.)& 0.5574 & 0.5550 & 0.9975 & 10\%\tabularnewline
I-FGSM (phys.)& 0.2284 & 0.2497 & 0.9453 & 95\%\tabularnewline
\hline 
\textbf{AdvNoise-DM (phys.)} & \textbf{0.0000} & \textbf{0.0000} & 0.6879 & \textbf{10\%}\tabularnewline
\textbf{$\text{MF}^{2}\text{M}$ (phys.)} & \textbf{0.0000} & \textbf{0.0000} & \textbf{0.6658} & \textbf{10\%}\tabularnewline
\hline 
\end{tabular}
}
\vspace{10pt}



\label{Table:physical_white}

\vspace{5pt}

\end{table}

==> FaceMask/table_black.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of each masking method on black-box attack.
``Rank 1'' refers to the top-1 identification rate and ``Veri.'' refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
   \begin{tabular}{l|ccc|ccc}
\hline 
 & \multicolumn{3}{c|}{CosFace ResNet50} & \multicolumn{3}{c}{CosFace ResNet34}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Face Rec. & \multicolumn{2}{c|}{\cellcolor{gray!40}Face Verification} & Face Rec. & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification}\tabularnewline
\cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
 & Rank 1 & Veri. & AUC & Rank 1 & Veri. & AUC\tabularnewline
\hline 
Solid-color & 0.8207 & 0.8233 & 0.9991 & 0.7641 & 0.7697 & 0.9987\tabularnewline
\hline 
FGSM & 0.7585 & 0.7624 & 0.9988 & 0.7147 & 0.7212 & 0.9984\tabularnewline
I-FGSM & 0.6720 & 0.6752 & 0.9978 & 0.6243 & 0.6303 & 0.9967\tabularnewline
MI-FGSM & 0.6419 & 0.6445 & 0.9972 & 0.6020 & 0.6077 & 0.9961\tabularnewline
TI-FGSM & 0.7640 & 0.7711 & 0.9988 & 0.7142 & 0.7214 & 0.9984\tabularnewline
TI-MI-FGSM & 0.6416 & 0.6438 & 0.9972 & 0.5996 & 0.6038 & 0.9958\tabularnewline
$\text{DI}^2$-FGSM & 0.7178 & 0.7222 & 0.9983 & 0.6699 & 0.6777 & 0.9977\tabularnewline
M-$\text{DI}^2$-FGSM & 0.6559 & 0.6592 & 0.9974 & 0.6165 & 0.6242 & 0.9963\tabularnewline
\hline 
\textbf{DM (ours)} & 0.6400 & 0.6520 & 0.9971 & 0.5987 & 0.6126 & 0.9971\tabularnewline
\textbf{AdvNoise-DM (ours)} & 0.0726 & 0.0723 & 0.9293 & 0.0657 & 0.0622 & 0.9310\tabularnewline
\textbf{$\text{MF}^2\text{M}$ (ours)} & \textbf{0.0674} & \textbf{0.0670} & \textbf{0.9237} & \textbf{0.0546} & \textbf{0.0508} & \textbf{0.9212}\tabularnewline
\hline 
\end{tabular}
}

\label{Table:table_black}

\vspace{5pt}

\end{table}

==> FaceMask/table_white.tex <==
\begin{table}[t]
% \footnotesize
% \scriptsize
    \centering
    % \vspace{-3pt}
    % \resizebox{\textwidth}{15mm}
    % \resizebox{1\linewidth}
    \caption{Multifaceted evaluation of each masking method on white-box attack. 
"Rank 1" refers to the top-1 identification rate and "Veri." refers to the TAR at $10^{-6}$ FAR.
}
    \vspace{-10pt}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l|cccc}
\hline 
 & \multicolumn{1}{c}{Face Rec.} & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification} & \multicolumn{1}{c}{Mask Detection}\tabularnewline
\cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5}
 & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Mask Rate} \tabularnewline
\hline 
Solid-color & 0.7389 & 0.7470 & 0.9986 & 90.53\%  \tabularnewline
\hline 
FGSM & 0.4895 & 0.4924 & 0.9950 & 62.10\%  \tabularnewline
I-FGSM & 0.0039 & 0.0026 & 0.7594 & 39.41\%  \tabularnewline
MI-FGSM & 0.0179 & 0.0135 & 0.8667 & 43.91\%  \tabularnewline
TI-FGSM & 0.4991 & 0.5053 & 0.9950 & 66.00\%  \tabularnewline
TI-MI-FGSM & 0.0364 & 0.0290 & 0.8998 & 51.97\%  \tabularnewline
$\text{DI}^2$-FGSM & 0.0690 & 0.0601 & 0.9193 & 43.51\%  \tabularnewline
M-$\text{DI}^2$-FGSM & 0.0705 & 0.0623 & 0.9293 & 45.50\% \tabularnewline
\hline
\textbf{DM (ours)} & 0.5146 & 0.5154 & 0.9956 & 27.74\%  \tabularnewline
\textbf{AdvNoise-DM (ours)} & \textbf{1.35$\text{e}^{-5}$} & \textbf{1.35$\text{e}^{-5}$} &  0.4163 & 7.30\% \tabularnewline
\textbf{$\text{MF}^2\text{M}$ (ours)} & \textbf{1.35$\text{e}^{-5}$} & 2.02$\text{e}^{-5}$ & \textbf{0.4093} & \textbf{6.95\%} \tabularnewline
\hline

%   \begin{tabular}{l|cccccc}
% \hline 
%  & \multicolumn{1}{c}{Face Recognition} & \multicolumn{2}{c}{\cellcolor{gray!40}Face Verification} & \multicolumn{1}{c}{Mask Detection} & \multicolumn{2}{c}{\cellcolor{gray!40}Similarity Metrics}\tabularnewline
% \cline{2-7} \cline{3-7} \cline{4-7} \cline{5-7} \cline{6-7} \cline{7-7} 
%  & \multicolumn{1}{c}{Rank 1} & \multicolumn{1}{c}{Veri.} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{Mask Rate} & \multicolumn{1}{c}{SSIM} & PSNR\tabularnewline
% \hline 
% Solid-color & 0.7389 & 0.7470 & 0.9986 & 90.53\% & —&— \tabularnewline
% \hline 
% FGSM & 0.4895 & 0.4924 & 0.9950 & 62.10\% & — & —\tabularnewline
% I-FGSM & 0.0039 & 0.0026 & 0.7594 & 39.41\% & — & — \tabularnewline
% MI-FGSM & 0.0179 & 0.0135 & 0.8667 & 43.91\% & — & — \tabularnewline
% TI-FGSM & 0.4991 & 0.5053 & 0.9950 & 66.00\% & — & — \tabularnewline
% TI-MI-FGSM & 0.0364 & 0.0290 & 0.8998 & 51.97\% & — & — \tabularnewline
% $\text{DI}^2$-FGSM & 0.0690 & 0.0601 & 0.9193 & 43.51\% &  — & — \tabularnewline
% M-$\text{DI}^2$-FGSM & 0.0705 & 0.0623 & 0.9293 & 45.50\% & — & —\tabularnewline
% \hline
% \textbf{DM (ours)} & 0.5146 & 0.5154 & 0.9956 & 27.74\% & — & — \tabularnewline
% \textbf{AdvNoise-DM} (ours) & \textbf{1.35$\text{e}^{-5}$} & \textbf{1.35$\text{e}^{-5}$} &  0.4163 & 7.30\% & 0.9808 & 38.76\tabularnewline
% \textbf{$\text{MF}^2\text{M}$} (ours) & \textbf{1.35$\text{e}^{-5}$} & 2.02$\text{e}^{-5}$ & \textbf{0.4093} & \textbf{6.95\%} & 0.9812 & 40.45 \tabularnewline
% \hline


\end{tabular}
}


\label{Table:table_white}

\vspace{5pt}

\end{table}
